MUSHY: Multimodal Flow-Based Amortized Bayesian Inference for Spectroscopic Data Fusion

We are in an era of unprecedented spectroscopic data availability, with surveys such as APOGEE, GALAH, and DESI observing millions of stars. However, data are heterogeneous and to date, efforts to exploit synergies between surveys have been limited. In particular, there is a lack of principled methods that combine spectroscopic data from different surveys to improve inference of physical parameters. In this work we present a new method, MUSHY, for spectroscopic data fusion. MUSHY is an amortized Bayesian inference method, using a rectified flow model with multimodal inputs to learn a posterior distribution over physical parameters. Using synthetic spectra generated via ATLAS12/SYNTHE, including realistic instrumental effects and noise, we demonstrate that MUSHY can precisely infer physical parameters with well-calibrated posteriors from any combination of surveys, with multimodal inputs providing stronger constraints on the posterior than single-survey data alone. This work paves the way for principled combination of spectroscopic data from heterogeneous sources.

==> architecture_spectra.tex <==
\begin{scope}[shift={(1.0,0.33)}, yscale=0.34]
  \draw[spec, apogee] plot coordinates {
      (0.0200,1.0000) (0.0234,1.0000) (0.0267,1.0000) (0.0301,0.9998) (0.0334,0.9993) (0.0368,0.9971) (0.0402,0.9903) (0.0435,0.9734)
      (0.0469,0.9396) (0.0503,0.8860) (0.0536,0.8215) (0.0570,0.7682) (0.0603,0.7502) (0.0637,0.7767) (0.0671,0.8343) (0.0704,0.8978)
      (0.0738,0.9464) (0.0771,0.9720) (0.0805,0.9728) (0.0839,0.9454) (0.0872,0.8826) (0.0906,0.7835) (0.0939,0.6675) (0.0973,0.5761)
      (0.1007,0.5517) (0.1040,0.6066) (0.1074,0.7136) (0.1108,0.8270) (0.1141,0.9133) (0.1175,0.9639) (0.1208,0.9874) (0.1242,0.9958)
      (0.1276,0.9968) (0.1309,0.9924) (0.1343,0.9805) (0.1376,0.9575) (0.1410,0.9231) (0.1444,0.8846) (0.1477,0.8562) (0.1511,0.8515)
      (0.1545,0.8727) (0.1578,0.9094) (0.1612,0.9462) (0.1645,0.9722) (0.1679,0.9832) (0.1713,0.9772) (0.1746,0.9494) (0.1780,0.8937)
      (0.1813,0.8115) (0.1847,0.7224) (0.1881,0.6606) (0.1914,0.6559) (0.1948,0.7105) (0.1982,0.7979) (0.2015,0.8830) (0.2049,0.9438)
      (0.2082,0.9775) (0.2116,0.9923) (0.2150,0.9968) (0.2183,0.9954) (0.2217,0.9874) (0.2250,0.9685) (0.2284,0.9342) (0.2318,0.8858)
      (0.2351,0.8357) (0.2385,0.8037) (0.2418,0.8056) (0.2452,0.8402) (0.2486,0.8909) (0.2519,0.9376) (0.2553,0.9678) (0.2587,0.9771)
      (0.2620,0.9618) (0.2654,0.9136) (0.2687,0.8245) (0.2721,0.7014) (0.2755,0.5782) (0.2788,0.5057) (0.2822,0.5193) (0.2855,0.6122)
      (0.2889,0.7405) (0.2923,0.8559) (0.2956,0.9336) (0.2990,0.9746) (0.3024,0.9916) (0.3057,0.9965) (0.3091,0.9947) (0.3124,0.9859)
      (0.3158,0.9660) (0.3192,0.9318) (0.3225,0.8866) (0.3259,0.8435) (0.3292,0.8208) (0.3326,0.8298) (0.3360,0.8659) (0.3393,0.9122)
      (0.3427,0.9518) (0.3461,0.9760) (0.3494,0.9830) (0.3528,0.9717) (0.3561,0.9381) (0.3595,0.8793) (0.3629,0.8032) (0.3662,0.7334)
      (0.3696,0.7004) (0.3729,0.7207) (0.3763,0.7840) (0.3797,0.8613) (0.3830,0.9262) (0.3864,0.9674) (0.3897,0.9880) (0.3931,0.9964)
      (0.3965,0.9991) (0.3998,0.9998) (0.4032,1.0000) (0.4066,1.0000) (0.4099,1.0000) (0.4133,1.0000) (0.4166,1.0000) (0.4200,1.0000)};
  \draw[spec, apogee] plot coordinates {
      (0.5000,1.0000) (0.5034,1.0000) (0.5067,1.0000) (0.5101,0.9998) (0.5134,0.9991) (0.5168,0.9965) (0.5202,0.9884) (0.5235,0.9681)
      (0.5269,0.9275) (0.5303,0.8632) (0.5336,0.7858) (0.5370,0.7219) (0.5403,0.7003) (0.5437,0.7320) (0.5471,0.8012) (0.5504,0.8776)
      (0.5538,0.9371) (0.5571,0.9716) (0.5605,0.9842) (0.5639,0.9798) (0.5672,0.9604) (0.5706,0.9277) (0.5739,0.8891) (0.5773,0.8587)
      (0.5807,0.8506) (0.5840,0.8689) (0.5874,0.9045) (0.5908,0.9420) (0.5941,0.9693) (0.5975,0.9812) (0.6008,0.9742) (0.6042,0.9416)
      (0.6076,0.8744) (0.6109,0.7721) (0.6143,0.6564) (0.6176,0.5701) (0.6210,0.5538) (0.6244,0.6157) (0.6277,0.7254) (0.6311,0.8372)
      (0.6345,0.9199) (0.6378,0.9673) (0.6412,0.9887) (0.6445,0.9959) (0.6479,0.9954) (0.6513,0.9878) (0.6546,0.9688) (0.6580,0.9333)
      (0.6613,0.8816) (0.6647,0.8255) (0.6681,0.7867) (0.6714,0.7837) (0.6748,0.8180) (0.6782,0.8729) (0.6815,0.9263) (0.6849,0.9640)
      (0.6882,0.9835) (0.6916,0.9880) (0.6950,0.9802) (0.6983,0.9609) (0.7017,0.9322) (0.7050,0.9021) (0.7084,0.8825) (0.7118,0.8830)
      (0.7151,0.9034) (0.7185,0.9337) (0.7218,0.9618) (0.7252,0.9798) (0.7286,0.9841) (0.7319,0.9708) (0.7353,0.9324) (0.7387,0.8618)
      (0.7420,0.7638) (0.7454,0.6647) (0.7487,0.6052) (0.7521,0.6143) (0.7555,0.6874) (0.7588,0.7898) (0.7622,0.8827) (0.7655,0.9457)
      (0.7689,0.9791) (0.7723,0.9929) (0.7756,0.9964) (0.7790,0.9931) (0.7824,0.9809) (0.7857,0.9537) (0.7891,0.9068) (0.7924,0.8442)
      (0.7958,0.7839) (0.7992,0.7515) (0.8025,0.7628) (0.8059,0.8122) (0.8092,0.8766) (0.8126,0.9328) (0.8160,0.9696) (0.8193,0.9886)
      (0.8227,0.9964) (0.8261,0.9991) (0.8294,0.9997) (0.8328,0.9992) (0.8361,0.9970) (0.8395,0.9898) (0.8429,0.9709) (0.8462,0.9313)
      (0.8496,0.8655) (0.8529,0.7814) (0.8563,0.7053) (0.8597,0.6703) (0.8630,0.6940) (0.8664,0.7644) (0.8697,0.8495) (0.8731,0.9203)
      (0.8765,0.9649) (0.8798,0.9872) (0.8832,0.9961) (0.8866,0.9990) (0.8899,0.9998) (0.8933,1.0000) (0.8966,1.0000) (0.9000,1.0000)};
  \draw[spec, apogee] plot coordinates {
      (0.9800,1.0000) (0.9834,1.0000) (0.9867,1.0000) (0.9901,0.9999) (0.9934,0.9994) (0.9968,0.9977) (1.0002,0.9922) (1.0035,0.9788)
      (1.0069,0.9517) (1.0103,0.9088) (1.0136,0.8572) (1.0170,0.8146) (1.0203,0.8002) (1.0237,0.8214) (1.0271,0.8675) (1.0304,0.9182)
      (1.0338,0.9569) (1.0371,0.9768) (1.0405,0.9756) (1.0439,0.9493) (1.0472,0.8905) (1.0506,0.7979) (1.0539,0.6896) (1.0573,0.6044)
      (1.0607,0.5816) (1.0640,0.6328) (1.0674,0.7327) (1.0708,0.8386) (1.0741,0.9191) (1.0775,0.9663) (1.0808,0.9883) (1.0842,0.9961)
      (1.0876,0.9969) (1.0909,0.9924) (1.0943,0.9805) (1.0976,0.9575) (1.1010,0.9231) (1.1044,0.8846) (1.1077,0.8562) (1.1111,0.8515)
      (1.1145,0.8727) (1.1178,0.9094) (1.1212,0.9463) (1.1245,0.9724) (1.1279,0.9841) (1.1313,0.9800) (1.1346,0.9565) (1.1380,0.9088)
      (1.1413,0.8384) (1.1447,0.7620) (1.1481,0.7091) (1.1514,0.7050) (1.1548,0.7518) (1.1582,0.8268) (1.1615,0.8997) (1.1649,0.9518)
      (1.1682,0.9807) (1.1716,0.9930) (1.1750,0.9955) (1.1783,0.9893) (1.1817,0.9687) (1.1850,0.9213) (1.1884,0.8355) (1.1918,0.7145)
      (1.1951,0.5891) (1.1985,0.5094) (1.2018,0.5139) (1.2052,0.6005) (1.2086,0.7276) (1.2119,0.8459) (1.2153,0.9276) (1.2187,0.9718)
      (1.2220,0.9906) (1.2254,0.9964) (1.2287,0.9952) (1.2321,0.9872) (1.2355,0.9686) (1.2388,0.9359) (1.2422,0.8913) (1.2455,0.8472)
      (1.2489,0.8218) (1.2523,0.8275) (1.2556,0.8615) (1.2590,0.9077) (1.2624,0.9490) (1.2657,0.9766) (1.2691,0.9910) (1.2724,0.9967)
      (1.2758,0.9971) (1.2792,0.9921) (1.2825,0.9776) (1.2859,0.9461) (1.2892,0.8924) (1.2926,0.8218) (1.2960,0.7552) (1.2993,0.7210)
      (1.3027,0.7362) (1.3061,0.7931) (1.3094,0.8653) (1.3128,0.9273) (1.3161,0.9674) (1.3195,0.9878) (1.3229,0.9960) (1.3262,0.9977)
      (1.3296,0.9953) (1.3329,0.9873) (1.3363,0.9703) (1.3397,0.9421) (1.3430,0.9063) (1.3464,0.8743) (1.3497,0.8601) (1.3531,0.8708)
      (1.3565,0.9010) (1.3598,0.9370) (1.3632,0.9668) (1.3666,0.9855) (1.3699,0.9947) (1.3733,0.9984) (1.3766,0.9996) (1.3800,0.9999)};
\end{scope}
\begin{scope}[shift={(1.0,-0.17)}, yscale=0.34]
  \draw[spec, galah] plot coordinates {
      (0.0000,1.0000) (0.0030,1.0000) (0.0061,1.0000) (0.0091,1.0000) (0.0121,0.9999) (0.0152,0.9994) (0.0182,0.9974) (0.0212,0.9912)
      (0.0242,0.9750) (0.0273,0.9406) (0.0303,0.8828) (0.0333,0.8076) (0.0364,0.7372) (0.0394,0.7011) (0.0424,0.7171) (0.0455,0.7772)
      (0.0485,0.8540) (0.0515,0.9203) (0.0545,0.9636) (0.0576,0.9854) (0.0606,0.9922) (0.0636,0.9886) (0.0667,0.9744) (0.0697,0.9481)
      (0.0727,0.9116) (0.0758,0.8747) (0.0788,0.8522) (0.0818,0.8549) (0.0848,0.8814) (0.0879,0.9194) (0.0909,0.9543) (0.0939,0.9780)
      (0.0970,0.9893) (0.1000,0.9890) (0.1030,0.9740) (0.1061,0.9354) (0.1091,0.8631) (0.1121,0.7581) (0.1152,0.6443) (0.1182,0.5646)
      (0.1212,0.5566) (0.1242,0.6241) (0.1273,0.7348) (0.1303,0.8443) (0.1333,0.9239) (0.1364,0.9691) (0.1394,0.9895) (0.1424,0.9970)
      (0.1455,0.9988) (0.1485,0.9979) (0.1515,0.9934) (0.1545,0.9816) (0.1576,0.9573) (0.1606,0.9172) (0.1636,0.8666) (0.1667,0.8210)
      (0.1697,0.8002) (0.1727,0.8143) (0.1758,0.8564) (0.1788,0.9076) (0.1818,0.9504) (0.1848,0.9773) (0.1879,0.9892) (0.1909,0.9883)
      (0.1939,0.9728) (0.1970,0.9358) (0.2000,0.8712) (0.2030,0.7847) (0.2061,0.7003) (0.2091,0.6529) (0.2121,0.6654) (0.2152,0.7316)
      (0.2182,0.8208) (0.2212,0.9004) (0.2242,0.9540) (0.2273,0.9823) (0.2303,0.9943) (0.2333,0.9984) (0.2364,0.9991) (0.2394,0.9978)
      (0.2424,0.9932) (0.2455,0.9819) (0.2485,0.9602) (0.2515,0.9270) (0.2545,0.8886) (0.2576,0.8586) (0.2606,0.8505) (0.2636,0.8686)
      (0.2667,0.9038) (0.2697,0.9414) (0.2727,0.9703) (0.2758,0.9875) (0.2788,0.9956) (0.2818,0.9987) (0.2848,0.9997) (0.2879,0.9999)
      (0.2909,1.0000) (0.2939,1.0000) (0.2970,1.0000) (0.3000,1.0000)};
  \draw[spec, galah] plot coordinates {
      (0.3700,1.0000) (0.3730,1.0000) (0.3761,1.0000) (0.3791,1.0000) (0.3821,0.9999) (0.3852,0.9996) (0.3882,0.9983) (0.3912,0.9941)
      (0.3942,0.9833) (0.3973,0.9604) (0.4003,0.9219) (0.4033,0.8718) (0.4064,0.8248) (0.4094,0.8007) (0.4124,0.8114) (0.4155,0.8515)
      (0.4185,0.9026) (0.4215,0.9468) (0.4245,0.9753) (0.4276,0.9883) (0.4306,0.9878) (0.4336,0.9718) (0.4367,0.9322) (0.4397,0.8616)
      (0.4427,0.7643) (0.4458,0.6659) (0.4488,0.6058) (0.4518,0.6130) (0.4548,0.6838) (0.4579,0.7850) (0.4609,0.8783) (0.4639,0.9427)
      (0.4670,0.9775) (0.4700,0.9927) (0.4730,0.9979) (0.4761,0.9991) (0.4791,0.9980) (0.4821,0.9939) (0.4852,0.9835) (0.4882,0.9629)
      (0.4912,0.9307) (0.4942,0.8923) (0.4973,0.8608) (0.5003,0.8501) (0.5033,0.8658) (0.5064,0.8999) (0.5094,0.9379) (0.5124,0.9678)
      (0.5155,0.9855) (0.5185,0.9921) (0.5215,0.9887) (0.5245,0.9721) (0.5276,0.9358) (0.5306,0.8759) (0.5336,0.7999) (0.5367,0.7315)
      (0.5397,0.7003) (0.5427,0.7215) (0.5458,0.7846) (0.5488,0.8614) (0.5518,0.9258) (0.5548,0.9669) (0.5579,0.9877) (0.5609,0.9961)
      (0.5639,0.9985) (0.5670,0.9973) (0.5700,0.9908) (0.5730,0.9719) (0.5761,0.9284) (0.5791,0.8479) (0.5821,0.7312) (0.5852,0.6047)
      (0.5882,0.5163) (0.5912,0.5073) (0.5942,0.5824) (0.5973,0.7054) (0.6003,0.8270) (0.6033,0.9153) (0.6064,0.9650) (0.6094,0.9858)
      (0.6124,0.9885) (0.6155,0.9775) (0.6185,0.9521) (0.6215,0.9124) (0.6245,0.8663) (0.6276,0.8303) (0.6306,0.8207) (0.6336,0.8423)
      (0.6367,0.8846) (0.6397,0.9297) (0.6427,0.9644) (0.6458,0.9850) (0.6488,0.9947) (0.6518,0.9985) (0.6548,0.9996) (0.6579,0.9999)
      (0.6609,1.0000) (0.6639,1.0000) (0.6670,1.0000) (0.6700,1.0000)};
  \draw[spec, galah] plot coordinates {
      (0.7300,1.0000) (0.7330,1.0000) (0.7361,1.0000) (0.7391,1.0000) (0.7421,0.9999) (0.7452,0.9996) (0.7482,0.9983) (0.7512,0.9941)
      (0.7542,0.9833) (0.7573,0.9604) (0.7603,0.9219) (0.7633,0.8718) (0.7664,0.8248) (0.7694,0.8007) (0.7724,0.8114) (0.7755,0.8515)
      (0.7785,0.9026) (0.7815,0.9469) (0.7845,0.9759) (0.7876,0.9909) (0.7906,0.9971) (0.7936,0.9991) (0.7967,0.9992) (0.7997,0.9975)
      (0.8027,0.9924) (0.8058,0.9803) (0.8088,0.9573) (0.8118,0.9232) (0.8148,0.8849) (0.8179,0.8564) (0.8209,0.8507) (0.8239,0.8705)
      (0.8270,0.9056) (0.8300,0.9408) (0.8330,0.9652) (0.8361,0.9757) (0.8391,0.9740) (0.8421,0.9628) (0.8452,0.9428) (0.8482,0.9135)
      (0.8512,0.8737) (0.8542,0.8223) (0.8573,0.7592) (0.8603,0.6860) (0.8633,0.6057) (0.8664,0.5233) (0.8694,0.4452) (0.8724,0.3783)
      (0.8755,0.3293) (0.8785,0.3033) (0.8815,0.3033) (0.8845,0.3293) (0.8876,0.3783) (0.8906,0.4452) (0.8936,0.5233) (0.8967,0.6057)
      (0.8997,0.6860) (0.9027,0.7592) (0.9058,0.8223) (0.9088,0.8737) (0.9118,0.9135) (0.9148,0.9427) (0.9179,0.9624) (0.9209,0.9727)
      (0.9239,0.9719) (0.9270,0.9560) (0.9300,0.9224) (0.9330,0.8749) (0.9361,0.8277) (0.9391,0.8011) (0.9421,0.8086) (0.9452,0.8465)
      (0.9482,0.8976) (0.9512,0.9431) (0.9542,0.9737) (0.9573,0.9899) (0.9603,0.9967) (0.9633,0.9989) (0.9664,0.9987) (0.9694,0.9957)
      (0.9724,0.9863) (0.9755,0.9638) (0.9785,0.9203) (0.9815,0.8540) (0.9845,0.7772) (0.9876,0.7171) (0.9906,0.7011) (0.9936,0.7372)
      (0.9967,0.8076) (0.9997,0.8828) (1.0027,0.9406) (1.0058,0.9750) (1.0088,0.9912) (1.0118,0.9974) (1.0148,0.9994) (1.0179,0.9999)
      (1.0209,1.0000) (1.0239,1.0000) (1.0270,1.0000) (1.0300,1.0000)};
  \draw[spec, galah] plot coordinates {
      (1.1000,1.0000) (1.1030,1.0000) (1.1061,1.0000) (1.1091,1.0000) (1.1121,0.9999) (1.1152,0.9995) (1.1182,0.9979) (1.1212,0.9927)
      (1.1242,0.9791) (1.1273,0.9505) (1.1303,0.9024) (1.1333,0.8397) (1.1364,0.7810) (1.1394,0.7509) (1.1424,0.7643) (1.1455,0.8143)
      (1.1485,0.8783) (1.1515,0.9336) (1.1545,0.9699) (1.1576,0.9886) (1.1606,0.9964) (1.1636,0.9989) (1.1667,0.9991) (1.1697,0.9975)
      (1.1727,0.9924) (1.1758,0.9803) (1.1788,0.9573) (1.1818,0.9232) (1.1848,0.8850) (1.1879,0.8566) (1.1909,0.8512) (1.1939,0.8716)
      (1.1970,0.9077) (1.2000,0.9448) (1.2030,0.9723) (1.2061,0.9873) (1.2091,0.9910) (1.2121,0.9825) (1.2152,0.9556) (1.2182,0.9010)
      (1.2212,0.8152) (1.2242,0.7129) (1.2273,0.6287) (1.2303,0.6004) (1.2333,0.6421) (1.2364,0.7332) (1.2394,0.8345) (1.2424,0.9146)
      (1.2455,0.9633) (1.2485,0.9869) (1.2515,0.9960) (1.2545,0.9987) (1.2576,0.9985) (1.2606,0.9953) (1.2636,0.9863) (1.2667,0.9662)
      (1.2697,0.9308) (1.2727,0.8822) (1.2758,0.8329) (1.2788,0.8029) (1.2818,0.8065) (1.2848,0.8419) (1.2879,0.8925) (1.2909,0.9392)
      (1.2939,0.9713) (1.2970,0.9888) (1.3000,0.9963) (1.3030,0.9988) (1.3061,0.9988) (1.3091,0.9962) (1.3121,0.9877) (1.3152,0.9669)
      (1.3182,0.9258) (1.3212,0.8614) (1.3242,0.7846) (1.3273,0.7215) (1.3303,0.7003) (1.3333,0.7315) (1.3364,0.7999) (1.3394,0.8759)
      (1.3424,0.9358) (1.3455,0.9721) (1.3485,0.9887) (1.3515,0.9921) (1.3545,0.9855) (1.3576,0.9678) (1.3606,0.9379) (1.3636,0.8999)
      (1.3667,0.8658) (1.3697,0.8501) (1.3727,0.8608) (1.3758,0.8923) (1.3788,0.9307) (1.3818,0.9629) (1.3848,0.9835) (1.3879,0.9939)
      (1.3909,0.9981) (1.3939,0.9995) (1.3970,0.9999) (1.4000,1.0000)};
\end{scope}
\begin{scope}[shift={(1.0,-0.67)}, yscale=0.34]
  \draw[spec, desi] plot coordinates {
      (0.0000,0.7200) (0.0088,0.7270) (0.0176,0.7337) (0.0264,0.7403) (0.0352,0.7467) (0.0440,0.7526) (0.0528,0.7572) (0.0616,0.7584)
      (0.0704,0.7515) (0.0792,0.7293) (0.0881,0.6858) (0.0969,0.6223) (0.1057,0.5542) (0.1145,0.5081) (0.1233,0.5067) (0.1321,0.5529)
      (0.1409,0.6279) (0.1497,0.7046) (0.1585,0.7633) (0.1673,0.7982) (0.1761,0.8117) (0.1849,0.8060) (0.1937,0.7804) (0.2025,0.7349)
      (0.2113,0.6772) (0.2201,0.6264) (0.2289,0.6047) (0.2377,0.6241) (0.2465,0.6770) (0.2553,0.7424) (0.2642,0.7994) (0.2730,0.8379)
      (0.2818,0.8582) (0.2906,0.8648) (0.2994,0.8617) (0.3082,0.8500) (0.3170,0.8301) (0.3258,0.8030) (0.3346,0.7721) (0.3434,0.7435)
      (0.3522,0.7244) (0.3610,0.7203) (0.3698,0.7332) (0.3786,0.7601) (0.3874,0.7949) (0.3962,0.8305) (0.4050,0.8613) (0.4138,0.8848)
      (0.4226,0.9008) (0.4314,0.9110) (0.4403,0.9172) (0.4491,0.9211) (0.4579,0.9238) (0.4667,0.9260) (0.4755,0.9277) (0.4843,0.9286)
      (0.4931,0.9275) (0.5019,0.9218) (0.5107,0.9080) (0.5195,0.8832) (0.5283,0.8492) (0.5371,0.8149) (0.5459,0.7939) (0.5547,0.7963)
      (0.5635,0.8216) (0.5723,0.8592) (0.5811,0.8957) (0.5899,0.9226) (0.5987,0.9387) (0.6075,0.9469) (0.6164,0.9507) (0.6252,0.9528)
      (0.6340,0.9542) (0.6428,0.9554) (0.6516,0.9565) (0.6604,0.9576) (0.6692,0.9586) (0.6780,0.9595) (0.6868,0.9602) (0.6956,0.9598)
      (0.7044,0.9568) (0.7132,0.9477) (0.7220,0.9282) (0.7308,0.8954) (0.7396,0.8527) (0.7484,0.8119) (0.7572,0.7893) (0.7660,0.7958)
      (0.7748,0.8285) (0.7836,0.8735) (0.7925,0.9150) (0.8013,0.9445) (0.8101,0.9612) (0.8189,0.9692) (0.8277,0.9726) (0.8365,0.9741)
      (0.8453,0.9749) (0.8541,0.9756) (0.8629,0.9762) (0.8717,0.9768) (0.8805,0.9774) (0.8893,0.9779) (0.8981,0.9785) (0.9069,0.9790)
      (0.9157,0.9795) (0.9245,0.9800) (0.9333,0.9804) (0.9421,0.9803) (0.9509,0.9791) (0.9597,0.9748) (0.9686,0.9641) (0.9774,0.9412)
      (0.9862,0.8999) (0.9950,0.8368) (1.0038,0.7559) (1.0126,0.6723) (1.0214,0.6084) (1.0302,0.5853) (1.0390,0.6112) (1.0478,0.6771)
      (1.0566,0.7619) (1.0654,0.8429) (1.0742,0.9059) (1.0830,0.9470) (1.0918,0.9700) (1.1006,0.9811) (1.1094,0.9859) (1.1182,0.9878)
      (1.1270,0.9886) (1.1358,0.9890) (1.1447,0.9894) (1.1535,0.9896) (1.1623,0.9899) (1.1711,0.9900) (1.1799,0.9899) (1.1887,0.9888)
      (1.1975,0.9853) (1.2063,0.9767) (1.2151,0.9603) (1.2239,0.9352) (1.2327,0.9057) (1.2415,0.8812) (1.2503,0.8721) (1.2591,0.8829)
      (1.2679,0.9085) (1.2767,0.9385) (1.2855,0.9634) (1.2943,0.9796) (1.3031,0.9880) (1.3119,0.9917) (1.3208,0.9931) (1.3296,0.9936)
      (1.3384,0.9939) (1.3472,0.9940) (1.3560,0.9942) (1.3648,0.9943) (1.3736,0.9945) (1.3824,0.9946) (1.3912,0.9947) (1.4000,0.9949)};
\end{scope}

